Leveraging Graph Diffusion Models for Network Refinement Tasks

Most real-world networks are noisy and incomplete samples from an unknown target distribution. Refining them by correcting corruptions or inferring unobserved regions typically improves downstream performance. Inspired by the impressive generative capabilities that have been used to correct corruptions in images, and the similarities between "in-painting" and filling in missing nodes and edges conditioned on the observed graph, we propose a novel graph generative framework, SGDM, which is based on subgraph diffusion. Our framework not only improves the scalability and fidelity of graph diffusion models, but also leverages the reverse process to perform novel, conditional generation tasks. In particular, through extensive empirical analysis and a set of novel metrics, we demonstrate that our proposed model effectively supports the following refinement tasks for partially observable networks: T1: denoising extraneous subgraphs, T2: expanding existing subgraphs and T3: performing "style" transfer by regenerating a particular subgraph to match the characteristics of a different node or subgraph.

==> ALGORITHMS/algorithm_figs.tex <==
\begin{figure}[t]
\begin{algorithm}[H]
\setstretch{1.1}
\caption{PreProcessing ~\OURS} 
\KwIn{$G = (\mA, \mX, \mE)$, $k$: the number of ego-net hops, $N_{max}$: maximum subgraph size, $d_{eigvec}$: dimension of global LPE} 
\KwOut{$\bm{\mathcal{S}}$: collection of ego-nets obtained from $G$} 
$\mL \gets \mI - \mD^{-\frac{1}{2}}\mA\mD^{-\frac{1}{2}}$ \Comment*[f]{$\mD$ is the diagonal degree matrix.}  \\ 
$\mQ \diag({\bm{\Lambda}}) \mQ \gets \text{EigenDecom}(\mL)$ \Comment*[f]{Compute Global Lap. Pos. Embed.} \\
$G \gets (\mA, \mX, \mE, \mQ[:,:d_{eigenvec}])$ \Comment*[f]{Add LPE to $G$.} \\
$\bm{\mathcal{S}} = \{\}$ \\
\For{i = 1 \KwTo $|\mX|$}{
    $N_i \gets  \text{K-Hop Neighbors}(i)$ \Comment*[f]{K-Hop Neighbors of Node $i$.} \\
    $S_i \gets \left(\mX[N_i], \mE[N_i], \mQ[N_i]\right)$ \Comment*[f]{Subgraph Induced by $N_i$.} \\
    $\bm{\mathcal{S}} \gets  S_i$ \Comment*[f]{Add to Set of Subgraphs.} \\
}
return $\bm{\mathcal{S}}$
\end{algorithm}\vspace{-0.10cm}

\begin{algorithm}[H]
\setstretch{1.1}
\caption{Training \OURS} \label{alg:trainingDiGress}
\KwIn{$\bm{\mathcal{S}} = \{S_1, \dots, S_{|\mX|}\}$: set of induced subgraphs. $\Omega_X$: transition matrix over node feature types X,$\Omega_E$: transition matrix over edge types}
Sample $t \sim \mathcal U(1, ..., T)$  \\
Sample $S_i(\mX_i, \mE_i, \mQ_i) \ \sim \bm{\mathcal{S}}$  \\
Sample $S_i^t(\overline{\mX}_i, \overline{\mE}_i) \sim \mX \Omega^t_X \times \tE \Omega^t_E$ \Comment*[f]{Sample a (discrete) noisy graph} \\
$z_i \gets  f(S_i^t, t)$ \Comment*[f]{Structural and spectral features} \\
$\hat p^X, \hat p^E \gets \phi_\theta(S_i^t, z_i, \mQ_i)$ 
\Comment*[f]{Forward pass, with global PE.} \\
$\operatorname{optimizer.step}(l_{CE}(\hat p^X, \mX) + \lambda ~ l_{CE}(\hat p^E, \tE))$ \Comment*[f]{Cross-entropy}\\

\end{algorithm}\vspace{-0.10cm}

\begin{algorithm}[H]
\setstretch{1.15}
\caption{Sampling from \OURS}\label{alg:SamplingDigress}
\KwIn{$\bm{\mathcal{M}} = \{ M_1 = (N_i,\dots N_j), \dots M_m = (N_m \dots N_n)\}$: node indices correponding to $m$ partitioned graphs obtained from $G$, where $\cap_1^m M_i = \emptyset$ and $\cup_1^m M_i = N$,$\Omega_X$, $\Omega_E$, $\mQ$} 

$\bm{\overline{\mathcal{M}}} = \{\} $\\
\For{$M_i$ \KwTo $\bm{\mathcal{M}}$}{
    $n \gets |M_i|$ \\
    Sample $\mX_i^T, \mY_i^T  \sim \Omega(n)_X \times \Omega(n)_E$ \Comment*[f]{Random graph}\\
    $\mQ_i\gets \mQ[M_i]$ \Comment*[f]{Corresponding Eigenvectors}\\
    $S^{t=T}_i \gets (\mX_i^T, \mE_i^T,\mQ_i) $  \\
    % TODO - Get p and q from a graph diffusion model \\
    \For{t = T \KwTo 1}{
        $z \gets  f(S_i^t, t)$ \Comment*[f]{Structural and spectral features} \\
        $\hat p^X, \hat p^E \gets \phi_\theta(S_i^t, z, \mQ_i)$
        \Comment*[f]{Forward pass} \\
        $ p_\theta(x^{t-1}_i | S_i^t) \gets \sum_x q(x_i^{t-1} | x_i=x, x_i^t) ~\hat p_i^X(x) \quad ~ i \in 1,\dots,n$ \Comment*[f]{Posterior}\\
        $ p_\theta(e^{t-1}_{ij} | S_i^t) \gets \sum_e q(e_{ij}^{t-1} | e_{ij}=e, e_{ij}^t)~ \hat p_{ij}^E(e) \quad ~ i,j \in 1,\dots,n$ \\
        $S^{t-1}_i \sim \prod_i p_\theta(x_i^{t-1} | S_i^t) \prod_{ij} p_\theta(e_{ij}^{t-1} | S_i^t)$ \Comment*[f]{Categorical distr.} 
    }
    $\bm{\overline{\mathcal{M}}} \gets S^{t=1}_i$ \\
}
$\overline{\mE} \gets \text{Coalesce}\left(\cup_{M_i(\mX_i, \mE_i,\mQ_i) \in \bm{\overline{\mathcal{M}}}}\mE_i\right)$ \Comment*[f]{Merge edges, drop duplicates.} \\
$\overline{\mX} \gets \text{Coalesce}\left(\cup_{M_i(\mX_i, \mE_i,\mQ_i) \in \bm{\overline{\mathcal{M}}}}\mX_i\right)$ \Comment*[f]{Merge nodes, drop duplicates.} \\
return $\overline{G}(\overline{\mX}, \overline{\mE})$
\end{algorithm}
\vspace{-0.4cm}
\caption{\textbf{Psuedocode for Training and Sampling.} We provide an illustrative example of how DiGress~\citep{digress_vignac22} can be straight-forwardly adapted to train on a single large network using $k$-hop ego-nets, positional encodings, and stitching.}

\end{figure}

\begin{figure}[t]

\begin{algorithm}[H]
\setstretch{1.1}
\caption{Expansion (Recovering Missing Edges) ~\OURS} 
\KwIn{$S\left(\mX, \mE, \mQ\right)$: subgraph that will be edited.} 
\KwOut{$\overline{S}\left(\overline{\mX}, \overline{\mE}, \overline{\mQ} \right)$: edited graph.} 
   $n \gets |S_i|$ \\
    Sample $\mX_i^T, \mE_i^T  \sim \Omega(n)_X \times \Omega(n)_E$ \Comment*[f]{Random graph}\\
    $S^{t=T}_i \gets (\mX_i^T, \mE_i^T,\mQ_i) $  \\
    \For{t = T \KwTo 1}{
        $z \gets  f(S_i^t, t)$ \Comment*[f]{Structural and spectral features} \\
        $\hat p^X, \hat p^E \gets \phi_\theta(S_i^t, z, \mQ_i)$
        \Comment*[f]{Forward pass} \\
        $ p_\theta(x^{t-1}_i | S_i^t) \gets \sum_x q(x_i^{t-1} | x_i=x, x_i^t) ~\hat p_i^X(x) \quad ~ i \in 1,\dots,n$ \Comment*[f]{Posterior}\\
        $ p_\theta(e^{t-1}_{ij} | S_i^t) \gets \sum_e q(e_{ij}^{t-1} | e_{ij}=e, e_{ij}^t)~ \hat p_{ij}^E(e) \quad ~ i,j \in 1,\dots,n$ \\
        $S^{t-1}_i \sim \prod_i p_\theta(x_i^{t-1} | S_i^t) \prod_{ij} p_\theta(e_{ij}^{t-1} | S_i^t)$ \Comment*[f]{Categorical distr.} \\
        $\mE_i^{t-1} \gets (1 - \mE) \odot \mE_i^{t-1} + \mE$ \Comment*[f]{"Repaint" with conditional edges.} \\
        $\mX_i^{t-1} \gets (1 - \mX) \odot \mX_i^{t-1} + \mX$ \Comment*[f]{"Repaint" with conditional feats.} \\
    }
    return $S^{t=1}_i(\mX^{t=1}_i, \mE^{t=1}_i, \mQ^{t=1}_i)$ 
\end{algorithm}\vspace{-0.10cm}
\caption{\textbf{Pseudocode for Editing.} Using a trained denoising model, we use a simple re-painting approach to recover missing edges given a starting or conditional subgraph.}
\end{figure}

\begin{figure}[t]

\begin{algorithm}[H]
\setstretch{1.1}
\caption{Denoising (Removing Noisy Edges) ~\OURS} 
\KwIn{$S\left(\mX, \mE, \mQ\right)$: subgraph that will be edited. $R$: number of concurrent trajectories; $W$: num of warm-up epochs} 
\KwOut{$\overline{S}\left(\overline{\mX}, \overline{\mE}, \overline{\mQ} \right)$: edited graph.} 
    $n \gets |S|$ \\
    $\mathcal{S} = \{\}$ \\ 
    \For{r = 1 \KwTo R}{
    Sample $\mX_r^T, \mE_r^T  \sim \Omega(n)_X \times \Omega(n)_E$ \Comment*[f]{Random graph}\\
    $S^{t=T}_r \gets (\mX_r^T, \mE_r^T,\mQ_i) $  \\
    $\mathcal{S} \gets S^{t=T}_r$  
    }
    \Comment*[f]{Guided Warm-up} \\ 
    
    \For{r = 1 \KwTo R}{
        \For{t = T \KwTo T-W}{
            $z \gets  f(S_r^t, t)$ \Comment*[f]{Structural and spectral features} \\
            $\hat p^X, \hat p^E \gets \phi_\theta(S_r^t, z, \mQ_r)$
            \Comment*[f]{Forward pass} \\
            $ p_\theta(x^{t-1}_r | S_r^t) \gets \sum_x q(x_r^{t-1} | x_r=x, x_r^t) ~\hat p_r^X(x) \quad ~ i \in 1,\dots,n$ \Comment*[f]{Posterior}\\
            $ p_\theta(e^{t-1}_{ij} | S_r^t) \gets \sum_e q(e_{ij}^{t-1} | e_{ij}=e, e_{ij}^t)~ \hat p_{ij}^E(e) \quad ~ i,j \in 1,\dots,n$ \\
            $S^{t-1}_r \sim \prod_i p_\theta(x_r^{t-1} | S_r^t) \prod_{ij} p_\theta(e_{ij}^{t-1} | S_r^t)$ \Comment*[f]{Categorical distr.} \\
            $\mE_r^{t-1} \gets (1 - \mE) \odot \mE_r^{t-1} + \mE$ \Comment*[f]{"Repaint" with conditional edges.} \\
            $\mX_r^{t-1} \gets (1 - \mX) \odot \mX_r^{t-1} + \mX$ \Comment*[f]{"Repaint" with conditional feats.} \\
        }
    } 
    \Comment*[f]{Probabilistic Masking} \\
    \For{t = T-W \KwTo 1}{
        \For{r = 1 \KwTo R}{
        $z \gets  f(S_i^t, t)$ \Comment*[f]{Structural and spectral features} \\
        $\hat p^X, \hat p^E \gets \phi_\theta(S_i^t, z, \mQ_i)$
        \Comment*[f]{Forward pass} \\
        $ p_\theta(x^{t-1}_i | S_i^t) \gets \sum_x q(x_i^{t-1} | x_i=x, x_i^t) ~\hat p_i^X(x) \quad ~ i \in 1,\dots,n$ \Comment*[f]{Posterior}\\
        $ p_\theta(e^{t-1}_{ij} | S_i^t) \gets \sum_e q(e_{ij}^{t-1} | e_{ij}=e, e_{ij}^t)~ \hat p_{ij}^E(e) \quad ~ i,j \in 1,\dots,n$ \\
        $S^{t-1}_i \sim \prod_i p_\theta(x_i^{t-1} | S_i^t) \prod_{ij} p_\theta(e_{ij}^{t-1} | S_i^t)$ \Comment*[f]{Categorical distr.} \\
        % $\mE_i^{t-1} \gets (1 - \mE) \odot \mE_i^{t-1} + \mE$ \Comment*[f]{"Repaint" with conditional edges.} \\
        % $\mX_i^{t-1} \gets (1 - \mX) \odot \mX_i^{t-1} + \mX$ \Comment*[f]{"Repaint" with conditional feats.} \\
        }
        \Comment*[f]{Compute the mask; add about the filtering step.}\\
        $\mE_i^{t-1}$ \\
        % $\mE_i^{t-1} \gets (1 - \mE) \odot \mE_i^{t-1} + \mE$ \Comment*[f]{"Repaint" with conditional edges.} \\
        % $\mX_i^{t-1} \gets (1 - \mX) \odot \mX_i^{t-1} + \mX$ \Comment*[f]{"Repaint" with conditional feats.} \\
    }
    return $S^{t=1}_i(\mX^{t=1}_i, \mE^{t=1}_i, \mQ^{t=1}_i)$ 
\end{algorithm}\vspace{-0.10cm}
\caption{\textbf{Pseudocode for Editing.} Using a trained denoising model, we will use multiple trajectories to model uncertainity over the substructure-based conditioning.}
\end{figure}

==> TABLES/edge_obs_struct.tex <==
\begin{table}[]
\centering
\caption{\textbf{Benefits of \ours.} Compared against EDGE, the only comparable single-graph GDDM, we see that using \ours improves performance. Note, that EDGE uses the degree distribution to guide the reverse process to improve scalability. This has negative effects on \texttt{T1:~Expansion}, as it constrains the model to satisfy an expected number of edges. Using other DM backbones helps resolve this problem.}
\label{tab:my-table}
\resizebox{\textwidth}{!}{%
\begin{tabular}{llllllrrrrr}
\toprule
Dataset &
  Task &
  Method &
  SGDM &
  Global-Context &
  Alignment &
  Conditioning &
  \multicolumn{1}{l}{Consensus} &
  \multicolumn{1}{l}{Diversity} &
  \multicolumn{1}{l}{Sparsity} &
  \multicolumn{1}{l}{Edge Overlap} \\
\midrule
BA-Shapes & Denoising & EDGE & \xmark  & \xmark  & \xmark  & Obs-Subst & 0.954 & 0.834 & 0.055  & 0.04273 \\
BA-Shapes & Denoising & EDGE & \checkmark & \xmark  & \xmark  & Obs-Subst & 0.751 &  0.992 & 0.364 & 0.3427 \\ 
\midrule
BA-Shapes & Denoising & EDGE & \xmark  & $\checkmark$ & $\checkmark$ & Obs-Subst & 0.996 & 0.733 & 0.019  & 0.01519 \\
BA-Shapes & Denoising & EDGE & $\checkmark$ & $\checkmark$ & \xmark  & Obs-Subst & 0.341 & 0.928 & 0.762  & 0.721   \\
\midrule
BA-Shapes & Expansion & EDGE & \xmark & \xmark  & \xmark  & Obs-Subst & 0.000 & 0.100 & 0.930 & 1.000 \\ 
BA-Shapes & Expansion & EDGE & $\checkmark$ & \xmark  & \xmark  & Obs-Subst & 0.055 & 0.1   & 0.93   & 1       \\
\midrule
BA-Shapes & Expansion & EDGE & \xmark  & $\checkmark$ & \xmark  & Obs-Subst & 0.000 & 0.100 & 0.930 & 1.000 \\
BA-Shapes & Expansion & EDGE & $\checkmark$ & $\checkmark$ & \xmark  & Obs-Subst & 0.055 & 0.1   & 0.93   & 1       \\
\midrule
Cora      & Denoising & EDGE & \xmark  & \xmark  & \xmark  & Obs-Subst & 0.916 & 0.915 & 0.115  & 0.0957  \\
Cora      & Denoising & EDGE & $\checkmark$ & \xmark  & $\checkmark$ & Obs-Subst & 0.587 & 1     & 0.591  & 0.58509 \\
\midrule
Cora      & Denoising & EDGE & \xmark  & $\checkmark$ & \xmark  & Obs-Subst & 0.965 & 0.798 & 0.057  & 0.04864 \\
Cora      & Denoising & EDGE & $\checkmark$ & $\checkmark$ & \xmark  & Obs-Subst & 0.754 & 1     & 0.442  & 0.43763 \\
\midrule
Cora      & Expansion & EDGE & \xmark  & \xmark  & \xmark  & Obs-Subst & 0     & 0.1   & 0.922  & 1       \\
Cora      & Expansion & EDGE & $\checkmark$ & \xmark  & \xmark  & Obs-Subst & 0     & 0.1   & 0.925  & 1       \\
\midrule
Cora      & Expansion & EDGE & \xmark  & $\checkmark$ & \xmark  & Obs-Subst & 0     & 0.1   & 0.922  & 1       \\
Cora      & Expansion & EDGE & $\checkmark$ & $\checkmark$ & \xmark  & Obs-Subst & 0     & 0.1   & 0.918  & 1       \\
\midrule
PolBlogs  & Denoising & EDGE & \xmark  & \xmark  & \xmark  & Obs-Subst & 0.992 & 0.702 & 0.0411 & 0.0412  \\
PolBlogs  & Denoising & EDGE & $\checkmark$ & \xmark  & \xmark  & Obs-Subst & 0.713 & 1     & 0.34   & 0.31515 \\
\midrule
PolBlogs  & Denoising & EDGE & \xmark  & $\checkmark$ & \xmark  & Obs-Subst & 0.993 & 0.598 & 0.023  & 0.02181 \\
PolBlogs  & Denoising & EDGE & $\checkmark$ & $\checkmark$ & \xmark  & Obs-Subst & 0.375 & 1     & 0.64   & 0.59266 \\
\midrule
PolBlogs  & Expansion & EDGE & \xmark  & \xmark  & \xmark  & Obs-Subst & 0     & 0.1   & 0.941  & 1.000       \\
PolBlogs  & Expansion & EDGE & $\checkmark$ & \xmark  & \xmark  & Obs-Subst & 0     & 0.1   & 0.939  & 1.000       \\
% \midrule
\midrule
PolBlogs  & Expansion & EDGE & \xmark  & $\checkmark$ & \xmark  & Obs-Subst & 0     & 0.1   & 0.938  & 1.000       \\
PolBlogs  & Expansion & EDGE & $\checkmark$ & $\checkmark$ & \xmark  & Obs-Subst & 0     & 0.1   & 0.939  & 1.000  \\
\bottomrule
\end{tabular}%
}
\end{table}

==> TABLES/evaluation_equations.tex <==
\begin{table}
\centering
\caption{\textbf{Graph Refinement Metrics.}} \label{table:metrics}
\resizebox{0.9\columnwidth}{!}{\begin{tabular}{ll}
\toprule
\textbf{Metric} & \textbf{Equation} \\
\midrule
Consensus & $\frac{1}{|\missingedge|}\sum_{[i,j] \in \missingedge}\frac{1}{R}\sum_{r=1}^R \mathds{1}\left[{\genedge}^r_{[i,j]} = {\targetedge}_{[i,j]}\right]$ \\
Edge Overlap & $\frac{1}{R}\sum_{r=1}^R \mathds{1}\left[{\genedge}^r\odot {\observededge}\right]$ \\
Diversity & $\frac{1}{R(R-1)}\sum_{r_1=1}^R \sum_{r_2=1}^R \mathds{1}\left[{\genedge}^{r_1} \neq {\genedge}^{r_2} \right]$\\
Density & $\frac{1}{R}\sum_{r=1}^R\frac{|\genedge^r|}{|\targetedge|}$\\
\bottomrule
\end{tabular}}
\end{table}

==> TABLES/recover_missing_edges_ba.tex <==
% \begin{table}[h!]
% \centering
% \caption{\textbf{Graph Denoising (Recovering Missing Edges), BA-Shapes.} Our variants are through row-sections 2-5, where row-section 5 corresponds to the test-time information baseline.$^1$: Graphs have been subsampled during generation.
% }
% \label{table:graph-denoising-adding-edges-results-ba}
% \vspace{-2mm}
% \footnotesize

% \resizebox{\textwidth}{!}{\begin{tabular}{l cccc}
% \toprule
% & 
% \textbf{Consensus} $(\uparrow)$ & \textbf{Diversity} $(\uparrow)$ & \textbf{Sparsity} $(\approxeq 1)$ & \textbf{Edge Overlap} $(\approxeq 1)$  
% \\
% \midrule
% % GraphMAE & 0.000 & 0.000 & 0.000 & 0.000 & 
% % 0.000 & 0.000 & 0.000 & 0.000  \\
% % GraphSAGE & 0.000 & 0.000 & 0.000 & 0.000 & 
% % 0.000 & 0.000 & 0.000 & 0.000  \\
% % VGAE & 0.000 & 0.000 & 0.000 & 0.000 & 
% % 0.000 & 0.000 & 0.000 & 0.000  \\
% % EDGE-Conditional & 0.000 & 0.000 & 0.000 & 0.000 & 
% % 0.000 & 0.000 & 0.000 & 0.000  \\
% % VGAE & 0.000 & 0.000 & 0.000 \\
% DRuM & 0.000 & 0.000 & 0.000 \\
% % EDGE-Unconditional 
% % EDGE-Subgraph Consolidated & 0.085 & $0.100^*$ & 1.316  \\
% EDGE-(Vanilla, Obs. Degree, No PE) & 0.085 & $0.100^*$ & 1.316  \\
% % EDGE-(Vanilla, Partition, Aligned) & 0.088 & $1.000$ & 0.484  \\
% EDGE-(Vanilla, Obs. Degree, PE) & 0.000 &  $0.100^*$ & 0.930   \\
% % EDGE-(Vanilla, Partition, PE, Aligned) &  &  &   \\
% \midrule
% \midrule
% EDGE-(Obs. Degree, No PE, Alignment) & 0.108 & \underline{0.996} & 0.485 & 0.143 \\ 
% EDGE-(Obs. Degree, PE, No Alignment) & 0.121 &  \underline{0.993} & 0.486 & 0.154 \\
% \midrule
% EDGE-(Obs. Degree, No PE, Subst.) & 0.055 & 0.100 & \underline{0.930} & NA \\ 
% EDGE-(Obs. Degree, PE, Subst.) & 0.055 &  0.100 & \underline{0.930} & NA\\ 
% \midrule
% DiGRESS-(PE, Subst.) & \underline{0.309} & 0.616 & \textbf{1.039} & NA \\
% DiGRESS-(PE, No Subst.) & \textbf{0.550} & \textbf{1.000} & 5.738 & NA  \\
% \midrule
% GDSS- (No PE, Subst)^1 & 0.325 &  0.977 & 1.532 \\
% GDSS- (PE, Subst) & & &  \\
% \midrule
% EDGE-(\textcolor{red}{Target} Degree, No PE, Subst.) & 0.589 & 0.511 & 1.002 & NA\\ 
% EDGE-(\textcolor{red}{Target} Degree, PE, Subst.) & 0.594 &  0.511 & 1.002 & NA \\ 
% % &  .000 & 0.000 & 0.000 & 0.000  \\
% \bottomrule
% \end{tabular}
% }
% \end{table}

% \begin{table}[h!]
% \centering
% \caption{\textbf{Graph Denoising (Recovering Missing Edges), CORA.} Our variants are through row-sections 2-5, where row-section 5 corresponds to the test-time information baseline.
% }
% \label{table:graph-denoising-adding-edges-results-cora}
% \vspace{-2mm}
% \footnotesize

% \resizebox{\textwidth}{!}{\begin{tabular}{l cccc}
% \toprule
% & 
% \textbf{Consensus} $(\uparrow)$ & \textbf{Diversity} $(\uparrow)$ & \textbf{Sparsity} $(\approxeq 1)$ & \textbf{Edge Overlap} $(\approxeq 1)$  
% \\
% \midrule
% EDGE-(Vanilla, Obs. Degree, No PE) & 0.005 &  0.171 & 0.991  & \\  
% EDGE-(Vanilla, Obs. Degree, No PE, Subst.) & 0.000 & 0.100 & 0.922 & \\  
% EDGE-(Vanilla, \textcolor{red}{Target} Degree, No PE, Subst.) & 0.020 & 0.520 & 0.944 & \\  
% % EDGE-(Vanilla, Partition, Aligned) & &  &  & \\  
% EDGE-(Vanilla, Obs. Degree, PE) & &  &  & \\  
% % EDGE-(Vanilla, Partition, PE, Aligned) &  &  &   \\
% \midrule
% \midrule
% EDGE-(Obs. Degree, No PE, Alignment) & 0.005 & 0.100 &  0.515 & 8.569 \\  
% EDGE-(Obs. Degree, PE, No Alignment) & &  &  & \\  
% \midrule
% EDGE-(Obs. Degree, No PE, Subst.) & &  &  & \\  
% EDGE-(Obs. Degree, PE, Subst.) & &  &  & \\  
% \midrule
% DiGRESS-(PE, Subst.) & 0.021 &  0.949 & 1.353 \\  
% DiGRESS-(PE, No Subst.) & &  &  & \\  
% \midrule
% GDSS- (No PE, Subst)^1 & & & \\
% GDSS- (PE, Subst) & & &  \\
% \midrule
% EDGE-(\pt{TARGET} Degree, No PE, Subst.) & 0.550 & 0.510 & 1.001 & 1.00 \\ 
% EDGE-(\pt{TARGET} Degree, PE, Subst.)& &  &  & \\
% % &  0.000 & 0.000 & 0.000 & 0.000  \\
% \bottomrule
% \end{tabular}
% }
% \end{table}



\begin{table}[h!]
\centering
\caption{\textbf{Graph Expansion, PolBlogs.} \pt{Convert to images for understanding.Add the runtimes.} --- break out gdss and digress into other tables -- start with EDGE, then show that its flexible to framework. Remove the target conditioning to the appendix. Simplify everything. Try making bar charts (Parittion vs. Non partition bar charts per metrics)   --- remove th
}
\label{table:graph-denoising-adding-edges-results-polblogs}
\vspace{-2mm}
\footnotesize

\resizebox{\textwidth}{!}{\begin{tabular}{l ccc ccccc}
\toprule
\textbf{Method} & \textbf{Partition?} & \textbf{PE?} & \textbf{Alignment?} & \textbf{Conditioning?} & \textbf{Consensus} $(\uparrow)$ & \textbf{Diversity} $(\uparrow)$ & \textbf{Sparsity} $(\approxeq 1)$ & \textbf{Edge Overlap} $(\approxeq 1)$  
\\
\midrule

\rowcolor{gray!50} EDGE	&	\xmark	&	\xmark	&	\checkmark	& Obs. Degree&	0.149	&	1.000 & 1.021 & -- \\	
EDGE	&	\xmark	&	\xmark	&	\xmark	& Obs. Degree + Subst.				&	0	&	0.100 & 0.941 & 1.000\\	
EDGE	&	\xmark	&	\xmark	&	\xmark	& \textcolor{red}{Target}	Degree	+	Subst.	&	0.046	&	0.909 & 0.998 & 1.000\\	
EDGE	&	\xmark	&	\checkmark	&	 \xmark	& Obs. Degree				&	0.129	&	1.000 & 1.012 & 0.155 \\	
EDGE	&	\xmark	&	\checkmark	&	\xmark	& Obs. Degree + Subst.				&	0	&	0.100 & 0.938 & 1.000 \\	
EDGE	&	\xmark	&	\checkmark	&	\xmark	&\textcolor{red}{Target}	Degree	+	Subst.	&	0.046	&	0.888 &  0.994 &  1.000 \\	
\midrule
EDGE & \checkmark & \xmark & \checkmark & Obs. Degree & 0.400 &  1.000 & 1.126 & 0.414 \\  
EDGE & \checkmark & \xmark & \xmark & Obs. Degree + Subst. & 0.000 &  0.100 & 0.939 & 1.000 \\  
EDGE & \checkmark & \xmark & \xmark & \textcolor{red}{Target} Degree + Subst.  & 0.681 &  0.363 &  1.002 & 1.000\\  

EDGE & \checkmark & \checkmark & \xmark & Obs. Degree & 0.135 & 1.000 & 1.095 & 0.251 \\  
EDGE & \checkmark & \checkmark & \xmark & Obs. Degree + Subst. & 0.000 & 0.100 & 0.939 & 1.000\\  
EDGE & \checkmark & \checkmark & \xmark & \textcolor{red}{Target} Degree + Subst. & 0.652 & 0.392 & 1.002 & 1.000 \\  
\midrule
GDSS & \checkmark & \xmark & \xmark &  Subst. & 0.217 & 1.000 & 5.444 & 1.000\\  
GDSS & \checkmark & \checkmark & \xmark &  Subst. & 0.305 & 1.000 & 14.174 & 1.000 \\  
\midrule
DiGRESS & \checkmark & \checkmark & \xmark &  Subst.  & 0.034 & 0.991 & 1.153 & 1.000 \\  
DiGRESS & \checkmark & \checkmark & \xmark & None & 0.031 & 0.994 & 1.134 & 1.000 \\  
\bottomrule
\end{tabular}
}
\end{table}




\begin{table}[h!]
\centering
\caption{\textbf{Graph Expansion, BA-Shapes.} Our variants are through row-sections 2-5, where row-section 5 corresponds to the test-time information baseline.$^1$: Graphs have been subsampled during generation.
}
\label{table:graph-denoising-adding-edges-results-ba}
\vspace{-2mm}
\footnotesize

\resizebox{\textwidth}{!}{\begin{tabular}{l ccc ccccc}
\toprule
 \textbf{Method} & \textbf{Partition?} & \textbf{PE?} & \textbf{Alignment?} & \textbf{Conditioning?} & \textbf{Consensus} $(\uparrow)$ & \textbf{Diversity} $(\uparrow)$ & \textbf{Sparsity} $(\approxeq 1)$ & \textbf{Edge Overlap} $(\approxeq 1)$  
\\
\midrule
\rowcolor{gray!50} EDGE & \xmark & \xmark & \checkmark & Obs. Degree & 0.085 & $0.100^*$ & 1.316  \\
EDGE & \xmark & \checkmark & \xmark & Obs. Degree  & 0.000 &  $0.100^*$ & 0.930   \\
\midrule
EDGE & \checkmark & \xmark & \checkmark & Obs. Degree & 0.108 & \underline{0.996} & 0.485 & 0.143 \\ 
EDGE & \checkmark & \xmark & \xmark & Obs. Degree + Subst. & 0.055 & 0.100 & \underline{0.930} & 1.000 \\ 
EDGE & \checkmark & \xmark & \xmark & \textcolor{red}{Target} Degree + Subst. & 0.589 & 0.511 & 1.002 & 1.000 \\ 
EDGE & \checkmark & \checkmark & \xmark & Obs. Degree & 0.121 &  \underline{0.993} & 0.486 & 0.154 \\
EDGE & \checkmark & \checkmark &  \xmark & Obs. Degree + Subst. & 0.055 &  0.100 & \underline{0.930} & 1.000 \\ 
EDGE & \checkmark & \checkmark & \xmark & \textcolor{red}{Target} Degree + Subst. & 0.594 &  0.511 & 1.002 & 1.000 \\ 
\midrule
GDSS & \checkmark & \xmark & \xmark & Subst.^1 & 0.296 & 0.983 & 1.707 & 1.000 \\
GDSS & \checkmark & \checkmark & \xmark &  Subst.^1 & 0.869 & 0.565 & 8.798 & 1.000\\
\midrule
DiGRESS & \checkmark & \checkmark & \xmark & Subst. & \underline{0.309} & 0.616 & \textbf{1.039} & 1.000 \\
DiGRESS & \checkmark & \checkmark & \xmark & None & \textbf{0.550} & \textbf{1.000} & 5.738 & 1.000  \\
\bottomrule
\end{tabular}
}
\end{table}


\begin{table}[h!]
\centering
\caption{\textbf{Graph Expansion (Recovering Missing Edges), CORA.}
}
\label{table:graph-denoising-adding-edges-results-cora}
\vspace{-2mm}
\footnotesize

\resizebox{\textwidth}{!}{\begin{tabular}{l ccc ccccc}
\toprule
 \textbf{Method} & \textbf{Partition?} & \textbf{PE?} & \textbf{Alignment?} & \textbf{Conditioning?} & \textbf{Consensus} $(\uparrow)$ & \textbf{Diversity} $(\uparrow)$ & \textbf{Sparsity} $(\approxeq 1)$ & \textbf{Edge Overlap} $(\approxeq 1)$  
\\
\midrule
% EDGE-(Vanilla, Obs. Degree, No PE) & 0.005 &  0.171 & 0.991  & \\  
% Consensus: 0.236, Diversity: 0.998, Sparsity: 0.358, Edge Overlap: 30.504
\rowcolor{gray!50} EDGE & \xmark & \xmark & \checkmark & Obs. Degree  & 0.236 &  0.998 & 0.358  & 0.305 \\  
EDGE & \xmark & \xmark & \xmark & Obs. Degree + Subst. & 0.000 & 0.100 & 0.922 & 1.00 \\  
EDGE & \xmark & \xmark &  \xmark & \textcolor{red}{Target} Degree + Subst. & 0.020 & 0.520 & 0.944 & 1.00 \\  
EDGE & \xmark & \checkmark & \checkmark & Obs. Degree  & 0.006 & 0.956 & 0.148 & 0.747 \\  
EDGE & \xmark & \checkmark  & \xmark & Obs. Degree + Subst. & 0.000 & 0.100 & 0.922 & 1.000\\  
EDGE & \xmark & \checkmark  &  \xmark & \textcolor{red}{Target} Degree + Subst. & 0.020 &  0.493 & 0.940 &  1.000 \\  
% EDGE-(Vanilla, Partition, Aligned) & &  &  & \\  
% EDGE-(Vanilla, Partition, PE, Aligned) &  &  &   \\
\midrule
EDGE & \checkmark & \xmark & \checkmark & Obs. Degree & 0.348 & 0.993 &  1.024 & 0.417 \\  
EDGE & \checkmark & \xmark & \xmark & Obs. Degree + Subst. & 0.000 & 0.100 & 0.925 & 1.00  \\  
EDGE & \checkmark & \xmark & \xmark & \textcolor{red}{Target} Degree + Subst. & 0.550 & 0.510 & 1.001 & 1.00 \\ 
EDGE & \checkmark & \checkmark & \xmark & Obs. Degree & 0.088 & 0.999 & 1.027 &  0.214 \\
EDGE & \checkmark & \checkmark & \xmark & Obs. Degree + Subst. & 0.000 & 0.100 & 0.918 & 1.000 \\ 
EDGE & \checkmark & \checkmark & \xmark & \textcolor{red}{Target} Degree + Subst. & 0.542 & 0.535 & 1.000 & 1.000 \\ 
\midrule
GDSS & \checkmark & \xmark & \xmark & Subst.^1 & 0.246 & 1.000 & 5.098 & 1.000 \\
GDSS & \checkmark & \checkmark & \xmark & Subst.^1 & 0.223 & 1.000 & 10.730 & 1.000 \\
\midrule
DiGRESS & \checkmark & \checkmark & \xmark & Subst. & 0.117 & 0.933 &  1.831 & 1.000 \\
DiGRESS & \checkmark & \checkmark & \xmark  & None & 0.142 & 0.968 &  1.755 & 1.000\\  
\bottomrule
\end{tabular}
}
\end{table}

==> TABLES/remove_extra_edges.tex <==
\begin{table}[h!]
\centering
\caption{\textbf{Graph Denoising (Removing Additional Edges), BA-Shapes.} 
}
\label{table:graph-denoising-removing-edges-results-bashapes}
\vspace{-2mm}
\footnotesize

\resizebox{\textwidth}{!}{\begin{tabular}{l cccc ccccc}
\toprule
\textbf{Method} & \textbf{Partition?} & \textbf{PE?} & \textbf{Alignment?} & \textbf{Subsampling?} & \textbf{Conditioning?} & \textbf{Consensus} $(\uparrow)$ & \textbf{Diversity} $(\uparrow)$ & \textbf{Sparsity} $(\approxeq 1)$ & \textbf{Edge Overlap} $(\approxeq 1)$  
\\
\midrule
% \rowcolor{gray!50} EDGE	&	\xmark	&	\xmark	&	\checkmark	& Obs. Degree &&  &  & \\  	
% EDGE	&	\xmark	&	\xmark	&	\xmark	& Obs. Degree + Subst. &	
% EDGE	&	\xmark	&	\xmark	&	\xmark	& \textcolor{red}{Target} Degree + Subst. &&  &  & \\  	
% EDGE	&	\xmark	&	\checkmark	&	 \xmark	& Obs. Degree & &  &  & \\  	
% EDGE	&	\xmark	&	\checkmark	&	\xmark	& Obs. Degree + Subst. &&  &  & \\  	
% EDGE	&	\xmark	&	\checkmark	&	\xmark	&\textcolor{red}{Target}	Degree	+	Subst.	&&  &  & \\  	
% \midrule
% EDGE & \checkmark & \xmark & \checkmark & Obs. Degree &&  &  & \\   
% EDGE & \checkmark & \xmark & \xmark & Obs. Degree + Subst. &&  &  & \\   
% EDGE & \checkmark & \xmark & \xmark & \textcolor{red}{Target} Degree + Subst.  &&  &  & \\   

% EDGE & \checkmark & \checkmark & \xmark & Obs. Degree &&  &  & \\   
% EDGE & \checkmark & \checkmark & \xmark & Obs. Degree + Subst. &&  &  & \\

%partition-bashapes, edge-add_nope_cheatcode_nosubsampling: Consensus: 0.723, Diversity: 0.992, Sparsity: 0.463, PreOverlap: 43.295, PostOverlap: nan
%partition-bashapes, edge-add_nope_degree-subst_nosubsampling: Consensus: 0.635, Diversity: 0.990, Sparsity: 0.462, PreOverlap: 43.091, PostOverlap: nan
% partition-bashapes, edge-add_nope_degreeonly_nosubsampling: Consensus: 0.924, Diversity: 1.000, Sparsity: 1.045, PreOverlap: 29.658, PostOverlap: 36.444

EDGE & \checkmark & \checkmark & \xmark & \checkmark & Obs. Degree & 0.772 & 1.000 & 1.074 &  0.3320 \\ 
EDGE  & \checkmark & \checkmark & \xmark & \checkmark & Obs. Degree + Subst. &  0.256 & 0.903 & 0.874 & 0.8212 \\
EDGE & \checkmark & \checkmark & \xmark & \checkmark & \textcolor{red}{Target} Degree + Subst. & 0.580 & 0.976 & 0.797 & 0.753 \\
\midrule
EDGE  & \checkmark & \checkmark & \xmark & \xmark & Obs. Degree & 0.794 & 1.000 & 1.052 & 0.2943 \\
EDGE & \checkmark & \checkmark & \xmark & \xmark & Obs. Degree + Subst. & 0.341 & 0.928 & 0.762  & 0.721 \\
EDGE & \checkmark & \checkmark & \xmark & \xmark & \textcolor{red}{Target} Degree + Subst. & 0.544 & 0.979 & 0.720 & 0.6838 \\ 
\midrule
% EDGE (reverse masking) & \xmark & \xmark & \checkmark & -- & \textcolor{red}{Target} Degree + Subst &  0.959 & 0.834 &  0.060 & 4.562 \\
% EDGE & \xmark & \checkmark & \checkmark & -- & Obs. Degree & 0.983 & 0.912 & 0.507 & 0.523 \\
% EDGE (reverse mask) & \xmark & \checkmark & \xmark & -- & \textcolor{red}{Target} Degree + Subst &  0.970 & 0.562 & 0.018 & 0.0197 \\ 
% \midrule
EDGE & \xmark & \xmark & \checkmark & \xmark & Obs. Degree &  0.994 & 0.982 & 0.723 & 0.36962 \\
EDGE & \xmark & \xmark & \xmark & \xmark & Obs. Degree + Subst. & 0.954 & 0.834 & 0.055 & 0.04273 \\
EDGE & \xmark & \xmark & \xmark & \xmark & \textcolor{red}{Target} Degree + Subst. &  0.950 & 0.852 & 0.063 & 0.04562 \\
\midrule
EDGE & \xmark & \checkmark & \checkmark & \xmark & Obs. Degree &  0.984 &  0.941 &  0.561 & 4.947 \\
EDGE & \xmark & \checkmark & \checkmark & \xmark & Obs. Degree + Subst. & 0.996 & 0.733 & 0.019 & 1.519 \\
EDGE & \xmark & \checkmark & \checkmark & \xmark & \textcolor{red}{Target} Degree + Subst. &  0.996 &  0.736 &  0.020 & 1.560 \\
\midrule
DiGRESS  & \checkmark  &\checkmark & \xmark & \xmark & Subst. & 0.184 &  0.589 & 0.914 & -- \\
DiGRESS   & \checkmark  &\checkmark & \xmark & \checkmark & Subst. & 0.007 & 0.239 & 1.016  & -- \\ 
DiGRESS  & \checkmark  &\checkmark & \xmark & \checkmark & No Subst. & 0.016 & 0.421 & 1.026 & -- \\
\bottomrule
\end{tabular}
}
\end{table}

\begin{table}[h!]
\centering
\caption{\textbf{Graph Denoising (Removing Additional Edges), PolBlogs.} 
}
\label{table:graph-denoising-removing-edges-results-polblogs}
\vspace{-2mm}
\footnotesize

\resizebox{\textwidth}{!}{\begin{tabular}{l cccc ccccc}
\toprule
\textbf{Method} & \textbf{Partition?} & \textbf{PE?} & \textbf{Alignment?} & \textbf{Subsampling?} & \textbf{Conditioning?} & \textbf{Consensus} $(\uparrow)$ & \textbf{Diversity} $(\uparrow)$ & \textbf{Sparsity} $(\approxeq 1)$ & \textbf{Edge Overlap} $(\approxeq 1)$  
\\
\midrule
EDGE & \checkmark & \xmark & \checkmark  & \xmark & Obs. Degree & 0.958 &  1.000 &  1.584 & 0.21998 \\
EDGE  & \checkmark & \xmark & \xmark & \xmark & Obs. Degree + Subst. &  0.713 &  1.000 &  0.340 &  0.31515  \\
EDGE & \checkmark & \xmark & \xmark & \xmark & \textcolor{red}{Target} Degree + Subst. & 0.605 & 1.000 & 0.437 &  0.4044 \\  
\midrule
EDGE & \checkmark & \xmark & \checkmark & \xmark & Obs. Degree  & 0.951 & 1.000 & 1.630 & --  \\ 
EDGE & \checkmark & \checkmark & \xmark & \xmark & Obs. Degree + Subst. &  0.375 & 1.000 &  0.640 & 0.59266 \\
EDGE & \checkmark & \checkmark  & \xmark & \xmark & \textcolor{red}{Target} Degree + Subst. & 0.469 &  1.000 &  0.686 & 0.6356 \\
\midrule
EDGE & \xmark & \checkmark & \checkmark & \xmark & Obs. Degree & 0.973 & 1.000 &  1.008 &  0.10785  \\
EDGE & \xmark & \checkmark & \xmark & \xmark & Obs. Degree + Subst. & 0.993 &  0.598 & 0.023 & 0.02181 \\
EDGE & \xmark & \checkmark & \xmark & \xmark & \textcolor{red}{Target} Degree + Subst. &  0.991 &  0.539 & 0.018 & 0.0170   \\
\midrule
EDGE & \xmark & \xmark & \checkmark & \xmark & Obs. Degree & 0.976 & 1.000 &  1.133 & 0.2586 \\  
EDGE & \xmark & \xmark & \xmark & \xmark & Obs. Degree + Subst. & 0.992 & 0.702 & 0.0411 & 0.0412 \\
EDGE & \xmark & \xmark & \xmark & \xmark & \textcolor{red}{Target} Degree + Subst. &  0.992 &  0.717 & 0.042 & 0.03972 \\
\midrule
DiGRESS   & \checkmark  &\checkmark & \xmark & \checkmark & Subst. &  0.8239 &  0.99603 & 0.60938  & -- \\ 
DiGRESS & \checkmark & \checkmark & \xmark  & \checkmark & No Subst. & 0.886 & 1.000 &  2.125 & 0.42513 \\
\bottomrule
\end{tabular}
}
\end{table}

\begin{table}[h!]
\centering
\caption{\textbf{Graph Denoising (Removing Additional Edges), CORA.} 
}
\label{table:graph-denoising-removing-edges-results-cora}
\vspace{-2mm}
\footnotesize

\resizebox{\textwidth}{!}{\begin{tabular}{l cccc ccccc}
\toprule
\textbf{Method} & \textbf{Partition?} & \textbf{PE?} & \textbf{Alignment?} & \textbf{Subsampling?} & \textbf{Conditioning?} & \textbf{Consensus} $(\uparrow)$ & \textbf{Diversity} $(\uparrow)$ & \textbf{Sparsity} $(\approxeq 1)$ & \textbf{Edge Overlap} $(\approxeq 1)$  
\\
\midrule
% \rowcolor{gray!50} EDGE	&	\xmark	&	\xmark	&	\checkmark	& Obs. Degree &&  &  & \\  	
% EDGE	&	\xmark	&	\xmark	&	\xmark	& Obs. Degree + Subst. &	
% EDGE	&	\xmark	&	\xmark	&	\xmark	& \textcolor{red}{Target} Degree + Subst. &&  &  & \\  	
% EDGE	&	\xmark	&	\checkmark	&	 \xmark	& Obs. Degree & &  &  & \\  	
% EDGE	&	\xmark	&	\checkmark	&	\xmark	& Obs. Degree + Subst. &&  &  & \\  	
% EDGE	&	\xmark	&	\checkmark	&	\xmark	&\textcolor{red}{Target}	Degree	+	Subst.	&&  &  & \\  	
% \midrule
% EDGE & \checkmark & \xmark & \checkmark & Obs. Degree &&  &  & \\   
% EDGE & \checkmark & \xmark & \xmark & Obs. Degree + Subst. &&  &  & \\   
% EDGE & \checkmark & \xmark & \xmark & \textcolor{red}{Target} Degree + Subst.  &&  &  & \\   

% EDGE & \checkmark & \checkmark & \xmark & Obs. Degree &&  &  & \\   
% EDGE & \checkmark & \checkmark & \xmark & Obs. Degree + Subst. &&  &  &
EDGE & \checkmark & \xmark & \checkmark & \xmark & Obs. Degree & 0.978 &  1.000 & 1.148 & 0.36186 \\
EDGE & \checkmark & \xmark & \checkmark & \xmark & Obs. Degree + Subst. & 0.587 & 1.000 &  0.591 & 0.58509 \\ 
EDGE & \checkmark & \xmark & \checkmark & \xmark & \textcolor{red}{Target} Degree + Subst. & 0.731 & 0.999 &  0.588 & 0.58188 \\
\midrule
EDGE & \checkmark & \checkmark & \xmark & \xmark & Obs. Degree & 0.960  & 1.000 & 1.117 & 0.17615 \\
EDGE & \checkmark & \checkmark & \xmark & \xmark & Obs. Degree + Subst. & 0.754 &  1.000 &  0.442 & 0.43763 \\
EDGE &  \checkmark & \checkmark & \xmark & \xmark & \textcolor{red}{Target} Degree + Subst. & 0.836 & 1.000 & 0.441 & 0.43677 \\
\midrule
EDGE & \xmark & \xmark & \checkmark & \xmark & Obs. Degree  & 1.000 &  0.999 &  0.424 &  0.27787 \\
EDGE & \xmark  & \xmark & \xmark & \xmark & Obs. Degree + Subst. & 0.916 & 0.915 & 0.115 &  0.09570 \\
EDGE & \xmark & \xmark & \xmark & \xmark & \textcolor{red}{Target} Degree + Subst. & 0.873 & 0.931 & 0.118 & 0.09387 \\
\midrule
EDGE & \xmark & \checkmark & \checkmark & \xmark & Obs. Degree & 0.999 & 0.994 & 0.171 & 0.893 \\ 
EDGE & \xmark  & \checkmark & \xmark & \xmark & Obs. Degree + Subst. & 0.965 & 0.798 & 0.057 & 0.04864 \\
EGDE  & \xmark & \checkmark & \xmark & \xmark & \textcolor{red}{Target} Degree + Subst. & 0.978 & 0.999 & 0.067 &  0.05109 \\
\midrule
% EDGE & \checkmark & \checkmark & \xmark & \xmark  & Obs. Degree & 0.959 & 1.000 &  1.123 &  0.17796 \\ 
\midrule
DiGRESS & \checkmark & \checkmark & \xmark & \checkmark & None & 0.402 & 0.998 & 2.546 & -- \\
DiGRESS & \checkmark & \checkmark & \xmark & \checkmark & Subst. & 0.438 & 0.874 & 0.865 & 0.82835 \\
\bottomrule
\end{tabular}
}
\end{table}
